Inpainting-based Video Compression in FullHD

Compression methods based on inpainting are an evolving alternative to classical transform-based codecs for still images. Attempts to apply these ideas to video compression are rare, since reaching real-time performance is very challenging. Therefore, current approaches focus on simplified frame-by-frame reconstructions that ignore temporal redundancies. As a remedy, we propose a highly efficient, real-time capable prediction and correction approach that fully relies on partial differential equations (PDEs) in all steps of the codec: Dense variational optic flow fields yield accurate motion-compensated predictions, while homogeneous diffusion inpainting is applied for intra prediction. To compress residuals, we introduce a new highly efficient block-based variant of pseudodifferential inpainting. Our novel architecture outperforms other inpainting-based video codecs in terms of both quality and speed. For the first time in inpainting-based video compression, we can decompress FullHD (1080p) videos in real-time with a fully CPU-based implementation, outperforming previous approaches by roughly one order of magnitude.

==> colours.tex <==
% custom colour scheme
\definecolor{colmint}{HTML}{8DD3C7}
\definecolor{colyellow}{HTML}{FFFFB3}
\definecolor{colorange}{HTML}{FDB462}
\definecolor{colred}{HTML}{FB8072}
\definecolor{colviolet}{HTML}{BEBADA}
\definecolor{colblue}{HTML}{80B1D3}
